A directed isoperimetric inequality with application to Bregman near neighbor lower bounds

Bregman divergences $D_\phi$ are a class of divergences parametrized by a convex function $\phi$ and include well known distance functions like $\ell_2^2$ and the Kullback-Leibler divergence. There has been extensive research on algorithms for problems like clustering and near neighbor search with respect to Bregman divergences, in all cases, the algorithms depend not just on the data size $n$ and dimensionality $d$, but also on a structure constant $\mu \ge 1$ that depends solely on $\phi$ and can grow without bound independently. In this paper, we provide the first evidence that this dependence on $\mu$ might be intrinsic. We focus on the problem of approximate near neighbor search for Bregman divergences. We show that under the cell probe model, any non-adaptive data structure (like locality-sensitive hashing) for $c$-approximate near-neighbor search that admits $r$ probes must use space $\Omega(n^{1 + \frac{\mu}{c r}})$. In contrast, for LSH under $\ell_1$ the best bound is $\Omega(n^{1+\frac{1}{cr}})$. Our new tool is a directed variant of the standard boolean noise operator. We show that a generalization of the Bonami-Beckner hypercontractivity inequality exists "in expectation" or upon restriction to certain subsets of the Hamming cube, and that this is sufficient to prove the desired isoperimetric inequality that we use in our data structure lower bound. We also present a structural result reducing the Hamming cube to a Bregman cube. This structure allows us to obtain lower bounds for problems under Bregman divergences from their $\ell_1$ analog. In particular, we get a (weaker) lower bound for approximate near neighbor search of the form $\Omega(n^{1 + \frac{1}{cr}})$ for an $r$-query non-adaptive data structure, and new cell probe lower bounds for a number of other near neighbor questions in Bregman space.

==> prelim.tex <==
\section{Statement of Results}
\label{sec:preliminaries}

\sverror{remove section 3. add reference to l1 lower bound in 1.1}

\subsection{Our Results}
\label{sec:our-results}

\paragraph{Lower bounds via $\ell_1$}
\label{sec:lower-bounds-via}

In Section~\ref{sec:reduct-from-hamm} we prove the following result via a reduction from corresponding lower bounds for the Hamming cube. 

\begin{theorem}
\label{thm:basic-lb}
For asymmetric and uniform Bregman divergences in $\reals^{2d}$ (where $d$ is $\Omega(\log n)$), any $t$-probe randomized data structure 
that returns an approximate nearest neighbor within a $c$ multiplicative factor and with constant success probability
must use space $n^{1 + \Omega(\frac{1}{ct})}$. 

The same lower bound holds for symmetric and decomposable Bregman divergences in $\reals^d$. 
\end{theorem}



\aanote{These bijections imply a collection of straightforward results
  for exact nearest neighbor, approximate nearest neighbor, LSH, etc
  using the results where both query and database come from the
  Hamming cube. Collecting them will be a literature survey chore, but
  needs to be done before a paper submission.}

\svnote{It might be useful to flesh out one or two of the corollaries,
  so we can see directly what kinds of lower bounds pop out. After
  all, the motivation for what follows is that we want a stronger
  bound, which begs the question, ``stronger than what''.}

\paragraph{Lower bounds via Fourier analysis}
\label{sec:lower-bounds-via-1}

In Sections \ref{sec:asymm-bregm-cube}, \ref{sec:analysis-r_p_1-p_2} and \ref{sec:from-hyperc-lower} we prove the main result of this paper, theorem \ref{thm:main}.
The proof proceeds in three parts. In Section~\ref{sec:asymm-bregm-cube} we introduce the asymmetric noise operator for functions on $\{0,1\}^n$ and establish its basic Fourier-analytic properties. In Section~\ref{sec:analysis-r_p_1-p_2} we prove an isoperimetric inequality for this noise operator. Finally, in Section~\ref{sec:from-hyperc-lower}, we use this isoperimetric inequality to show the desired cell probe lower bound, by adapting the framework of \citet*{geometric}.





